On Feasibility of Declarative Diagnosis

The programming language Prolog makes declarative programming possible, at least to a substantial extent. Programs may be written and reasoned about in terms of their declarative semantics. All the advantages of declarative programming are however lost when it comes to program debugging. This is because the Prolog debugger is based solely on the operational semantics. Declarative methods of diagnosis (i.e. locating errors in programs) exist, but are neglected. This paper discusses their possibly main weaknesses and shows how to overcome them. We argue that useful ways of declarative diagnosis of logic programs exist, and should be usable in actual programming.

==> eptcsdata.tex <==
\providecommand{\firstpage}{193}
\providecommand{\publicationstatus}{S. Costantini, E. Pontelli, A. Russo, F. Toni,\\R. Calegari, A. D'Avila Garcez, C. Dodaro, F. Fabiano,\\ S. Gaggl, A. Mileo, (Eds.): ICLP 2023\\
EPTCS 385, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.385.20}{10.4204/EPTCS.385.20}}
\pdfoutput=1

